Chatting with a Learning Analytics Dashboard: The Role of Generative AI Literacy on Learner Interaction with Conventional and Scaffolding Chatbots

Learning analytics dashboards (LADs) simplify complex learner data into accessible visualisations, providing actionable insights for educators and students. However, their educational effectiveness has not always matched the sophistication of the technology behind them. Explanatory and interactive LADs, enhanced by generative AI (GenAI) chatbots, hold promise by enabling dynamic, dialogue-based interactions with data visualisations and offering personalised feedback through text. Yet, the effectiveness of these tools may be limited by learners' varying levels of GenAI literacy, a factor that remains underexplored in current research. This study investigates the role of GenAI literacy in learner interactions with conventional (reactive) versus scaffolding (proactive) chatbot-assisted LADs. Through a comparative analysis of 81 participants, we examine how GenAI literacy is associated with learners' ability to interpret complex visualisations and their cognitive processes during interactions with chatbot-assisted LADs. Results show that while both chatbots significantly improved learner comprehension, those with higher GenAI literacy benefited the most, particularly with conventional chatbots, demonstrating diverse prompting strategies. Findings highlight the importance of considering learners' GenAI literacy when integrating GenAI chatbots in LADs and educational technologies. Incorporating scaffolding techniques within GenAI chatbots can be an effective strategy, offering a more guided experience that reduces reliance on learners' GenAI literacy.

==> 8_supplementary_material.tex <==
\newpage
\section{Scaffolding Prompts and Questions}
\subsection{Scaffolding Prompts}
\textbf{Scaffolding Approach.} Guide participants through understanding each visualisation step-by-step. For each visualisation, start by providing a one-sentence description and ask only one question at a time. Avoid asking repeated questions. Give feedback on participants' responses. Once all questions for one visualisation are covered, direct participants to the next visualisation by asking them to click the right arrow. Only ask questions related to the visualisation that was sent to you. Ensure you cover all the \textbf{Scaffolding Questions} for each visualisation, including 1 for the Bar Chart, 2 for the Communication Network, and 3 for the Ward Map. Use a friendly and conversational tone. If participants get something wrong, provide a hint and ask them to rethink and re-answer. 

\subsection{Visualisation Descriptions and Scaffolding Questions}
\noindent\textbf{Bar Chart}
\begin{itemize}
    \item \textbf{Description:} It shows the proportion of time the two nurses spent on different tasks.
    \item \textbf{Scaffolding Question:}
    \begin{enumerate}
        \item What do you notice about Amy's proportion of time spent on tasks, and what does this indicate about her prioritisation?
    \end{enumerate}
\end{itemize}

\noindent\textbf{Communication Network}
\begin{itemize}
    \item \textbf{Description:} It shows verbal communication interactions among each student and their communication with the doctor, relative, and patient manikins. Arrows indicate the direction of communication, and edge thickness indicates the duration of communication.
    \item \textbf{Scaffolding Questions:}
    \begin{enumerate}
        \item Who are the main communicators in the network, and what does the thickness of the arrows tell us?
        \item How often did the nurses communicate with each other compared to the doctor, patient, and relative?
    \end{enumerate}
\end{itemize}

\noindent\textbf{Ward Map}
\begin{itemize}
    \item \textbf{Description:} It shows the verbal and spatial distribution of each student during a simulation session. Saturated colours indicate frequent verbal communication, while the hexagons' locations show spatial distributions. The peak heart rate of each student is also displayed on the Ward Map, represented by a heart shape.
    \item \textbf{Scaffolding Questions:}
    \begin{enumerate}
        \item Which areas of the ward did the nurses spend the most time in, and how does that relate to their task prioritisation?
        \item How can the colour intensity give us insights into verbal communication patterns?
        \item What does the peak heart rate tell us about the stress levels of the nurses in different areas of the ward?
    \end{enumerate}
\end{itemize}
